A comparison of matrix-free isogeometric Galerkin and collocation methods for Karhunen--Lo\`eve expansion

Numerical computation of the Karhunen--Lo\`eve expansion is computationally challenging in terms of both memory requirements and computing time. We compare two state-of-the-art methods that claim to efficiently solve for the K--L expansion: (1) the matrix-free isogeometric Galerkin method using interpolation based quadrature proposed by the authors in [1] and (2) our new matrix-free implementation of the isogeometric collocation method proposed in [2]. Two three-dimensional benchmark problems indicate that the Galerkin method performs significantly better for smooth covariance kernels, while the collocation method performs slightly better for rough covariance kernels.

==> sections/algorithms/algorithm1.tex <==
\begin{algorithm}
\textbf{Input}:
	$v_{i_1\ldots i_d} \in \mathbb{R}^{n_1 \times \cdots \times n_d}$,
	$J_{l_1\ldots l_d} \in \mathbb{R}^{\tilde{n}_1 \times \cdots \times \tilde{n}_d}$,
	$B_{i_k j_k} \in \mathbb{R}^{\tilde{n}_k \times \tilde{n}_k}$ and
	$M_{l_k j_k} \in \mathbb{R}^{\tilde{n}_k \times n_k}$\\
\textbf{Output}: $v^\prime_{i_1\dots i_d} \in \mathbb{R}^{n_1\times \cdots \times n_d}$
\begin{algorithmic}[1]
	\State $V_{j_1\ldots j_d} 		\leftarrow L^{-1}_{ i_1  j_1}\cdots L^{-1}_{ i_d  j_d} v_{ i_1\ldots i_d }$	\Comment{Preconditioning}
	\State $X_{k_1\ldots k_d} 	\leftarrow M_{k_1 j_1}\cdots M_{k_d j_d} V_{j_1\ldots j_d}$
	\State $Y_{l_1\ldots l_d} 	\leftarrow \invinterpmat{ k_1}{l_1 }\cdots \invinterpmat{ k_d}{l_d } X_{k_1\ldots k_d}$	\Comment{Using $\mat L \mat U$ fac.}
	\State $Y^\prime_{l_1\ldots l_d} \leftarrow J_{l_1\ldots l_d} \odot Y_{l_1\ldots l_d}$
	\State $Z^\prime_{k_1\ldots k_d} \leftarrow {\hat \Gamma}_{ k_1\ldots k_d l_1\ldots l_d} Y^\prime_{l_1\ldots l_d}$		\Comment{No forming of $\mat{\Gamma}$}
	\State $Z_{k_1\ldots k_d} \leftarrow J_{k_1\ldots k_d} \odot Z^\prime_{k_1\ldots k_d}$
	\State $Y_{j_1\ldots j_d} \leftarrow \invinterpmat{ j_1 }{  k_1 }\cdots \invinterpmat{ j_d }{ k_d } Z_{k_1\ldots k_d}$ 	\Comment{Using $\mat L \mat U$ fac. }
	\State $V_{l_1\ldots l_d} \leftarrow M_{j_1 l_1}\cdots M_{j_d l_d} Y_{j_1\ldots j_d}$
	\State $v_{i_1\ldots i_d}^\prime \leftarrow L^{-1}_{i_1 l_1}\cdots L^{-1}_{i_d l_d} V_{l_1\ldots l_d}$
  \Comment{Preconditioning}
\caption{Matrix-free evaluation of the matrix-vector product $\mat{v}^\prime \mapsto \mat{\tilde{A}}^\prime \mat{v}^\prime $}\label{alg:mf_eval}
\end{algorithmic}
\end{algorithm}

